Error Estimates and Physics Informed Augmentation of Neural Networks for Thermally Coupled Incompressible Navier Stokes Equations

Physics Informed Neural Networks (PINNs) are shown to be a promising method for the approximation of Partial Differential Equations (PDEs). PINNs approximate the PDE solution by minimizing physics-based loss functions over a given domain. Despite substantial progress in the application of PINNs to a range of problem classes, investigation of error estimation and convergence properties of PINNs, which is important for establishing the rationale behind their good empirical performance, has been lacking. This paper presents convergence analysis and error estimates of PINNs for a multi-physics problem of thermally coupled incompressible Navier-Stokes equations. Through a model problem of Beltrami flow it is shown that a small training error implies a small generalization error. Posteriori convergence rates of total error with respect to the training residual and collocation points are presented. This is of practical significance in determining appropriate number of training parameters and training residual thresholds to get good PINNs prediction of thermally coupled steady state laminar flows. These convergence rates are then generalized to different spatial geometries as well as to different flow parameters that lie in the laminar regime. A pressure stabilization term in the form of pressure Poisson equation is added to the PDE residuals for PINNs. This physics informed augmentation is shown to improve accuracy of the pressure field by an order of magnitude as compared to the case without augmentation. Results from PINNs are compared to the ones obtained from stabilized finite element method and good properties of PINNs are highlighted.

==> Deep_Feed_Forward_Neural_Networks.tex <==
\section{Deep Feed Forward Neural Networks for Solving PDEs} \label{Sec: DeepFeedNNforPDEs}
    As discussed in the previous section, within the context of approximate solution to PDE, a Neural Network (NN) is the representation of a trial nonlinear function. The structure of such NN consists of an input-layer followed by one or more internal layers ending with an output layer and each layer consists of neurons. For the input layer the neurons are typically the spatial-temporal location of the domain points. For example, the input layer for a two-dimensional spatial domain \((x,y)\) will consist of two inputs or neurons \({\bf{X}}=\{x,y\}\). The internal layers (also known as hidden layers) can have a variable number of neurons. These neurons represent the unknown functions used in building the WRM trial approximation while the output layer neurons contain the trial function values. The values of any layer i in the network can be represented in an algebraic form as follows:
    \begin{equation}\label{eq:1}
    {{\bf{z}}_i} = \sigma \left( {{{\bf{W}}_i}{{\bf{z}}_{i - 1}} + {{\bf{b}}_i}} \right) \quad {\rm{for}} \quad 1 \le i \le m
    \end{equation}
    and the values in the output layer are computed as:
    \begin{equation}\label{eq:2}
    {\bf{Y}} = \sigma \left( {{{\bf{W}}_{m + 1}}{{\bf{z}}_m} + {{\bf{b}}_{m + 1}}} \right)
    \end{equation}
    where \(m\) is the total number of hidden layers, \(\bf{W}\) is the tensor for weights, \(\bf{b}\) is the bias vector, \(\bf{Y}\) is the output vector, and \(\sigma\) is the activation function that acts as a transfer function to propagate data in the network. We have used hyperbolic tangent as an activation function in our framework. DNN approximates outputs by finding optimal weights and biases during the training process that minimizes an objective or loss function.
    
    In the context of solving general PDEs using DNN, let us consider a second order PDE in one-dimensional domain \(\Omega\) with non-homogeneous Dirichlet boundary conditions on its boundary \(\Gamma  = \partial \Omega\).
    \begin{equation}\label{eq:3}
    \mathcal{L}u\left( x \right) = f \quad \rm{on} \;  \Omega\\
    \end{equation}
    \begin{equation}\label{eq:4}
    u\left( x \right) = g \quad \rm{on} \; \Gamma
    \end{equation}
    where \(\mathcal{L}\) is the differential operator, \(u\)is the unknown solution field, and \(f\) is the source term. The loss function comprises of the governing equation which is based on physical laws.
    \begin{equation}\label{eq:5}
    {\rm{Loss}} = \mathcal{R} = \left\| { \mathcal{L}\hat u\left( {x;\bf{W,b}} \right) - f} \right\|_\Omega ^2 + \left\| { \hat u\left( {x;\bf{W,b}} \right) - g} \right\|_\Gamma ^2
    \end{equation}
    where \(\hat u\left( {x;\bf{W,b}} \right)\) is the DNN approximation to the solution \(u\left( x \right)\). Eq. \ref{eq:5} yields a constrained optimization problem in which the residual is minimized using optimization strategies such as the stochastic gradient descent methods during the training process:
    \begin{equation}\label{eq:6}
     \left\{{{\hat{\bf{W}},\hat{\bf{b}}}} \right\} = \argmin_{{\bf{W}},{\bfb}} \mathcal{\{R\}}
    \end{equation}
    where \(\hat{\bf{W}} {\rm{and}}\: {\hat{\bf{b}}}\) are optimized weights and biases, respectively, and are used by the DNN to approximate the PDE solution.
